"Gauge" in General Relativity: Second-order general relativistic gauge-invariant perturbation theory

As in the case of the other gauge field theories, there is so called ``gauge'' also in general relativity. This ``gauge'' is unphysical degree of freedom. There are two kinds of ``gauges'' in general relativity. These are called the first- and the second-kind of gauges, respectively. The gauge of the first kind is just coordinate system on a single manifold. On the other hand, the gauge of the second kind arises in the general relativistic perturbations. Through the precise distinction of these two concepts of ``gauges'', we develop second-order gauge-invariant general relativistic perturbation theory.

==> README <==
This directory contains four .sty files that are mutually compatible,
but actually independent:

cite.sty       Compressed, sorted lists of numerical citations: [8,11-16]

overcite.sty   Compressed, sorted lists of superscript numerical citations:
               "word [12,16,11,13,14,15]."  -->  "word.$^{11-16}$"

drftcite.sty   Print the tags instead of the numbers for \cite and \bibitem.

chapterbib.sty Do multiple bibliographies--one for each \include file.

Each package works with LaTeX2e and LaTeX2.09.  (These versions are the
last that will support 2.09!)  The documentation is included as plain
text after the definitions in each file (below \endinput).  It can be
read online or printed directly, but don't try to typeset it with LaTeX!

Since the instructions follow \endinput, they are not read by TeX and
should not slow down the file loading.  If, however, you see that the
instructions slow down the loading on your system, you may split the
file into, for example, cite.sty and cite.doc.  Just do not redistribute
these split files.

Donald Arseneau                         asnd@reg.triumf.ca

